Event-QA: A Dataset for Event-Centric Question Answering over Knowledge Graphs

Semantic Question Answering (QA) is a crucial technology to facilitate intuitive user access to semantic information stored in knowledge graphs. Whereas most of the existing QA systems and datasets focus on entity-centric questions, very little is known about these systems' performance in the context of events. As new event-centric knowledge graphs emerge, datasets for such questions gain importance. In this paper, we present the Event-QA dataset for answering event-centric questions over knowledge graphs. Event-QA contains 1000 semantic queries and the corresponding English, German and Portuguese verbalizations for EventKG - an event-centric knowledge graph with more than 970 thousand events.

==> 01_Introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Knowledge graphs (KGs) with popular examples including DBpedia \cite{dbpedia-swj}, Wikidata \cite{Vrandecic:2012}, YAGO \cite{RebeleSHBKW16} and EventKG \cite{Gottschalk:2018, GottschalkD19} have recently evolved as an important source of semantic information on the Web. 
%
Semantic Question Answering (QA) is a key technology
to facilitate intuitive access to knowledge graphs for end-users
via natural language (NL) interfaces. 
QA systems automatically translate a user question expressed in a natural language into the SPARQL query language to query knowledge graphs \cite{TrivediMDL17, lcquad2}.
%
In recent years, researchers have developed a large variety of QA approaches \cite{HoffnerWMULN17}. 


QA datasets play an essential role in the development and evaluation of QA systems \cite{lcquad2, UsbeckGN018}.
The active development of QA datasets supports the advancement of QA technology, for example, through the QALD (Question Answering over Linked Data) initiative\footnote{Question Answering over Linked Data: \url{http://qald.aksw.org}}. 
%
As popular knowledge graphs are mostly entity-centric, they do not sufficiently cover events and temporal relations \cite{Gottschalk:2018}. As a consequence, existing QA datasets, with recent examples including LC-QuAD \cite{TrivediMDL17}, LC-QuAD 2.0 \cite{lcquad2} and the QALD challenges, mainly focus on entity-centric queries.
%
More recently, event-centric knowledge graphs such as EventKG \cite{Gottschalk:2018} that includes historical and important contemporary events as well as knowledge graphs that contain daily happenings extracted from the news (e.g., \cite{Leetaru:2013, RospocherEVFARS16}) evolved. However, there is a lack of QA datasets dedicated to event-centric questions and only a few datasets (e.g., TempQuestions \cite{TempQuestions} and the dataset proposed by Saquete et al. \cite{SaqueteGMML09}) focus on temporal expressions.
This way, development and evaluation of QA systems concerning the event-centric questions are currently not adequately supported.

In this paper, we introduce novel \textit{Event-QA} (Event-Centric Question Answering Dataset) dataset for training and evaluating QA systems on complex event-centric questions over knowledge graphs. 
With complex, we mean that the intended SPARQL queries consist of more than one triple pattern, similar to \cite{TrivediMDL17}. %
The aims of \textit{Event-QA} are to: 
1) Provide a representative selection of relations involving events in the knowledge graph, to ensure the diversity of the resulting event-centric semantic queries. To achieve this goal, we approach the query generation via a random walk through the knowledge graph, starting from randomly selected relations.
2) Ensure the quality of the natural language questions. 
To this extent, the resulting queries are manually translated into natural language expressions in English, Portuguese and German.
%
To the best of our knowledge, this is the first QA dataset focused on event-centric questions so far, and the only QA dataset that targets EventKG.

The contributions of this paper are as follows: 
\begin{itemize}
\item We propose an approach for an automatic generation of semantic queries for an event-centric QA dataset from a knowledge graph. 
%
\item We present the \textit{Event-QA} dataset containing 3000 event-centric natural language questions (i.e. 1000 in each language) with the corresponding SPARQL interpretations for the EventKG knowledge graph. These questions exhibit a variety of SPARQL queries and their verbalizations.
%
To facilitate an easier integration with the existing QA pipelines, we also provide a translation of the SPARQL queries in \textit{Event-QA} to DBpedia, where possible.
%
\item We provide an open source, extensible framework for automatic dataset generation to facilitate dataset maintenance and updates.  
\end{itemize}

The remainder of the paper is organised as follows: In Section \ref{sec:relevance}, we discuss the motivation for an event-centric QA dataset. Then, in Section \ref{sec:problem}, we present the problem of the event-centric QA dataset generation. In Section \ref{sec:approach}, we describe the corresponding approach to generate an event-centric QA dataset from a knowledge graph. Following that, in Section \ref{sec:implementation}, we provide a brief overview of EventKG and the application of the proposed approach to this knowledge graph. Section \ref{sec:evaluation} discusses the characteristics of the resulting \textit{Event-QA} dataset, and Section \ref{sec:availability} summarises the availability aspects. Then, Section \ref{sec:related} gives an overview of the related work. Finally, Section \ref{sec:conclusion} provides a conclusion. 

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

